Cross-modal feature fusion for robust point cloud registration with ambiguous geometry

Point cloud registration has seen significant advancements with the application of deep learning techniques. However, existing approaches often overlook the potential of integrating radiometric information from RGB images. This limitation reduces their effectiveness in aligning point clouds pairs, especially in regions where geometric data alone is insufficient. When used effectively, radiometric information can enhance the registration process by providing context that is missing from purely geometric data. In this paper, we propose CoFF, a novel Cross-modal Feature Fusion method that utilizes both point cloud geometry and RGB images for pairwise point cloud registration. Assuming that the co-registration between point clouds and RGB images is available, CoFF explicitly addresses the challenges where geometric information alone is unclear, such as in regions with symmetric similarity or planar structures, through a two-stage fusion of 3D point cloud features and 2D image features. It incorporates a cross-modal feature fusion module that assigns pixel-wise image features to 3D input point clouds to enhance learned 3D point features, and integrates patch-wise image features with superpoint features to improve the quality of coarse matching. This is followed by a coarse-to-fine matching module that accurately establishes correspondences using the fused features. We extensively evaluate CoFF on four common datasets: 3DMatch, 3DLoMatch, IndoorLRS, and the recently released ScanNet++ datasets. In addition, we assess CoFF on specific subset datasets containing geometrically ambiguous cases. Our experimental results demonstrate that CoFF achieves state-of-the-art registration performance across all benchmarks, including remarkable registration recalls of 95.9% and 81.6% on the widely-used 3DMatch and 3DLoMatch datasets, respectively...(Truncated to fit arXiv abstract length)

==> equations/coarse_matching.tex <==
\begin{equation}
  \mathbf{\Omega}^\mathrm{c} = \{(\mathbf{p}^{\mathrm{s}}_{m_{j}},\mathbf{q}^{\mathrm{s}}_{n_{j}}) \mid (m_{j},n_{j}) \in \mathbf{\psi}(\mathbf{f}^\mathrm{*}_{\mathbf{P}}, \mathbf{f}^\mathrm{*}_{\mathbf{Q}}) \}.
  \label{eq:coarse_matching}
\end{equation}
where $(m_{j},n_{j})$ is a set of indices of coarse correspondences,

==> equations/fine_matching.tex <==
\begin{equation}
  \mathbf{\Omega}^\mathrm{f}_i = \{(\mathbf{p}^{\mathrm{d}}_{m_{j}},\mathbf{q}^{\mathrm{d}}_{n_{j}}) \mid (m_{j},n_{j}) \in \mathbf{\tau}({\mathbf{F}}^{\mathrm{3D}}_{\mathbf{P}},\mathbf{F}^{\mathrm{3D}}_{\mathbf{Q}}) \}.
  \label{eq:fine_matching}
\end{equation}
where $(m_{j},n_{j})$ is a set of indices of fine correspondences,

==> equations/first_fuse.tex <==
\begin{equation}
  \mathbf{F}^{\mathrm{*}}_{\mathbf{P}} = [\mathbf{F}^{\mathrm{2D}}_{\mathbf{P}},\mathbf{1}].
  \label{eq:first_fuse}
\end{equation}



==> equations/mapping.tex <==
\begin{equation}
  (u_{i, k}, v_{i, k}, z_i)^T = \mathbf{K} \cdot \mathbf{E}_k \cdot [x_i, y_i, z_i, 1]^T.
  \label{eq:project}
\end{equation}
\begin{equation}
  \mathbf{\pi}: \mathbb{R}^{2} \ni (u_{i, k}, v_{i, k}) \mapsto (x_i, y_i, z_i) \in \mathbb{R}^{3}
  \label{eq:mapping}
\end{equation}

==> equations/patch_feat_extract.tex <==
\begin{equation}
% \begin{aligned}
  \mathbf{f}^{\mathrm{2D}}_{\mathbf{P}} = \mathcal{E} ^{\mathrm{2D}}_2(\mathrm{resize}(\varphi(\mathbf{I}^{\mathrm{2}}_{\mathbf{P}}))), \\
  % & \mathbf{I}^{\mathrm{2}}_{\mathbf{P}} \in \mathbb{R}^{M^{\mathrm{s}} \times L \times H_{\mathrm{2}} \times W_{\mathrm{2}} \times C} \stackrel{\mathbf{\varphi}}{\longrightarrow} \mathbb{R}^{M^{\mathrm{s}} \times H_{\mathrm{2}} \times W_{\mathrm{2}} \times C}  \\
  % & \qquad \stackrel{\mathrm{resize}}{\longrightarrow} \mathbb{R}^{M^{\mathrm{s}} \times H_{\mathrm{2}}^0 \times W^0_{\mathrm{2}} \times C} \stackrel{\mathcal{E} ^{\mathrm{2D}}_2}{\longrightarrow} \mathbb{R}^{M^{\mathrm{s}} \times D_{\mathrm{2}}} \ni \mathbf{f}^{\mathrm{2D}}_{\mathbf{P}},
  % \end{aligned}
  \label{eq:patch_feat}
\end{equation}

==> equations/pixel_feat_extract.tex <==
\begin{equation}
    \mathbf{F}^{\mathrm{2D}}_{\mathbf{P}} = \phi(\mathbf{\pi}(\mathcal{E}^{\mathrm{2D}}_1(\mathbf{I}_{\mathbf{P}}))), 
  \label{eq:pixel_feat}
\end{equation}
where $\phi$ denotes the pixel-wise feature selection described in the subsequent multi-view feature fusion. $D_{\mathrm{1}}$ represents the dimensions of the extracted pixel-wise features. The feature $\mathbf{F}^{\mathrm{2D}}_{\mathbf{Q}}$ for $\mathbf{Q}$ is computed in a same way.

==> equations/ppt_equations.tex <==

\hat{\mathbf{F}}^{\mathbf{P}, \mathrm{2D}} \; \mathrm{or} \; \hat{\mathbf{F}}^{\mathbf{Q}, \mathrm{2D}}

\mathbf{F}^{\mathbf{Q},\mathrm{2D}}

\{\mathbf{P};\mathbf{F}^{\mathbf{P},\mathrm{input}}\}

\{\mathbf{Q};\mathbf{F}^{\mathbf{Q},\mathrm{input}}\}

\{\mathbf{P};\mathbf{F}^{\mathbf{P},\mathrm{fuse}}\}

\{\mathbf{Q};\mathbf{F}^{\mathbf{Q},\mathrm{fuse}}\}

\{\hat{\mathbf{P}};\hat{\mathbf{F}}^{\mathbf{P}, \mathrm{3D}}\}

\{\hat{\mathbf{Q}};\hat{\mathbf{F}}^{\mathbf{Q}, \mathrm{3D}}\}

\{\tilde{\mathbf{P}};\tilde{\mathbf{F}}^{\mathbf{P}, \mathrm{3D}}\}

\{\tilde{\mathbf{Q}};\tilde{\mathbf{F}}^{\mathbf{Q}, \mathrm{3D}}\}

\mathrm{Coarse \; matching} \; \hat{\mathbf{\Omega}}: \{\hat{\mathbf{F}}^{\mathbf{P},\mathrm{fuse}},\hat{\mathbf{F}}^{\mathbf{Q},\mathrm{fuse}}\}

\mathrm{Fine \; matching} \; \tilde{\mathbf{\Omega}}: \{\tilde{\mathbf{F}}^{\mathbf{Q},\mathrm{3D}},\tilde{\mathbf{F}}^{\mathbf{Q},\mathrm{3D}}\}

\{\mathbf{R},\mathbf{t}\}


==> equations/second_fuse.tex <==
\begin{equation}
  \mathbf{f}^\mathrm{*}_{\mathbf{P}} = \mathrm{MLP}([\mathbf{f}^\mathrm{3D}_{\mathbf{P}}, \mathbf{f}^{\mathrm{2D}}_{\mathbf{P}}]).
  \label{eq:second_fuse}
\end{equation}
% \vspace{-2mm}

==> figs/tex/pipeline.tex <==
\begin{figure}[tb]
  \centering
  \includegraphics[height=6.5cm]{figs/figure/eijkel2.pdf}
  \caption{Overview of our 2D-3D feature fusion pipeline. \textBF{Extractor} denotes }
  \label{fig:example}
\end{figure}

==> figs/tex/short.tex <==
\begin{figure}[tb]
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Centered, short example caption}
  \label{fig:short}
\end{figure}

==> secs/rest.tex <==
%%%%%%%%%%%%%%%%%%%%%
\section{Methodology}
\label{sec:method}

\subsection{2D-3D projection}
\label{sub_sec:projection}

\begin{equation}
  \mathbf{u} = \mathbf{K} \cdot \mathbf{M}_{\rm mount} \cdot \mathbf{M}_{\rm COP}^{-1} \cdot \mathbf{M}_{\rm SOP}^{-1} \cdot \mathbf{X}_{\rm PRCS},
  \label{eq:projection}
\end{equation}
where $\mathbf{u}$ denotes homogeneous image coordinates and $\mathbf{X}_{\rm PRCS}$ homogeneous point coordinates in project coordinate system (PRCS). $K$ denotes intrinsic matrix.

\begin{equation}
  (\mathbf{R^{\ast}},\mathbf{t^{\ast}}) = 
  \underset{(\mathbf{R},\mathbf{t}) \in SO(3) \times \mathbb{R}^3}{\mathrm{argmin}}{\sum\nolimits_{(\mathbf{p}_{m_{j}},\mathbf{q}_{n_{j}}) \in \overline{\mathbf{\Omega}}}{\left \| \mathbf{R} \cdot \mathbf{p}_{m_{j}} + \mathbf{t} - \mathbf{q}_{n_{j}} \right \|}^2_2},
  \label{eq:transform}
\end{equation}
where $\overline{\mathbf{\Omega}} = \{(\mathbf{p}_{m_{j}},\mathbf{q}_{n_{j}}) \mid j = 1, ..., O\}$ denotes the ground-truth correspondences.


\begin{algorithm}
\caption{Coarse-to-fine matching}
\label{algorithm}
\textbf{Input:} Description of the input parameters \\
\textbf{Output:} Description of the output 
\begin{algorithmic}[1]
    \STATE Extract patch-wise features for all points in $\mathbf{P}$ and $\mathbf{Q}$
    \STATE Pre-process the input data if needed
    \FOR{each element in the input data}
        \STATE Perform specific operation on the element
        \STATE Update variables/data structures if necessary
    \ENDFOR
    \WHILE{condition is true}
        \STATE Perform specific operations
        \STATE Check and update the condition
    \ENDWHILE
    \IF{specific condition is met}
        \STATE Execute corresponding operations
    \ELSE
        \STATE Execute alternative operations
    \ENDIF
    \STATE Post-process the results if needed
    \STATE \textbf{Return} the final result
\end{algorithmic}
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%
\section{Experiments}
\label{sec:experiments}

%%%%%%%%%%%%%%%%%%%%%
\section{Results}
\label{sec:results}

%%%%%%%%%%%%%%%%%%%%%
\section{Conclusion}
\label{sec:conclusion}

\subsection{Example Subsection}
\label{subsec1}

Subsection text.

%% Use \subsubsection, \paragraph, \subparagraph commands to 
%% start 3rd, 4th and 5th level sections.
%% Refer following link for more details.
%% https://en.wikibooks.org/wiki/LaTeX/Document_Structure#Sectioning_commands

\subsubsection{Mathematics}
%% Inline mathematics is tagged between $ symbols.
This is an example for the symbol $\alpha$ tagged as inline mathematics.

%% Displayed equations can be tagged using various environments. 
%% Single line equations can be tagged using the equation environment.
\begin{equation}
f(x) = (x+a)(x+b)
\end{equation}

%% Unnumbered equations are tagged using starred versions of the environment.
%% amsmath package needs to be loaded for the starred version of equation environment.
\begin{equation*}
f(x) = (x+a)(x+b)
\end{equation*}

%% align or eqnarray environments can be used for multi line equations.
%% & is used to mark alignment points in equations.
%% \\ is used to end a row in a multiline equation.
\begin{align}
 f(x) &= (x+a)(x+b) \\
      &= x^2 + (a+b)x + ab
\end{align}

\begin{eqnarray}
 f(x) &=& (x+a)(x+b) \nonumber\\ %% If equation numbering is not needed for a row use \nonumber.
      &=& x^2 + (a+b)x + ab
\end{eqnarray}

%% Unnumbered versions of align and eqnarray
\begin{align*}
 f(x) &= (x+a)(x+b) \\
      &= x^2 + (a+b)x + ab
\end{align*}

\begin{eqnarray*}
 f(x)&=& (x+a)(x+b) \\
     &=& x^2 + (a+b)x + ab
\end{eqnarray*}

%% Refer following link for more details.
%% https://en.wikibooks.org/wiki/LaTeX/Mathematics
%% https://en.wikibooks.org/wiki/LaTeX/Advanced_Mathematics

%% Use a table environment to create tables.
%% Refer following link for more details.
%% https://en.wikibooks.org/wiki/LaTeX/Tables
\begin{table}[t]%% placement specifier
%% Use tabular environment to tag the tabular data.
%% https://en.wikibooks.org/wiki/LaTeX/Tables#The_tabular_environment
\centering%% For centre alignment of tabular.
\begin{tabular}{l c r}%% Table column specifiers
%% Tabular cells are separated by &
  1 & 2 & 3 \\ %% A tabular row ends with \\
  4 & 5 & 6 \\
  7 & 8 & 9 \\
\end{tabular}
%% Use \caption command for table caption and label.
\caption{Table Caption}\label{fig1}
\end{table}


%% Use figure environment to create figures
%% Refer following link for more details.
%% https://en.wikibooks.org/wiki/LaTeX/Floats,_Figures_and_Captions
\begin{figure}[t]%% placement specifier
%% Use \includegraphics command to insert graphic files. Place graphics files in 
%% working directory.
\centering%% For centre alignment of image.
\includegraphics{example-image-a}
%% Use \caption command for figure caption and label.
\caption{Figure Caption}\label{fig2}
%% https://en.wikibooks.org/wiki/LaTeX/Importing_Graphics#Importing_external_graphics
\end{figure}

==> tabs/abla_color_methods.tex <==
\begin{table}[tb]
  \setlength{\tabcolsep}{4pt}
  \renewcommand{\arraystretch}{1.2}
  \caption{Comparison between different color assisted methods on 3DMatch and 3DLoMatch.}
  \vspace{-1em}
  \label{tab:abla_color_methods}
  \centering
  \resizebox{\columnwidth}{!}{
  \begin{tabular}{l|ccc|ccc}
    \toprule
     & \multicolumn{3}{c|}{3DMatch}&  \multicolumn{3}{c}{3DLoMatch}\\
    \midrule
    Method & FMR (\%)$\uparrow$ & IR (\%)$\uparrow$ & RR (\%)$\uparrow$ & FMR (\%)$\uparrow$ & IR (\%)$\uparrow$ & RR (\%)$\uparrow$ \\
    % \midrule
    \midrule
    Color ICP~\cite{Park2017}~&~xx~&~xx~&~xx~~~&~~xx~&~xx~&~xx~\\
    LCD~\cite{pham2020lcd}~&~xxx~&~xx~&~xx~~~&~~xx~&~xx~&~xx~\\   
    PCR-CG(retrain)~&~97.1~&~57.4~&~90.6~~~&~~80.5~&~28.1~&~65.6~\\    Ours~&~\textBF{99.5}~&~\underline{74.3}~&~\textBF{95.9}~~~&~~\textBF{93.6}~&~\textBF{47.4}~&~\textBF{81.6}~\\
    Color ICP + ours~&~xxx~&~xx~&~xx~~~&~~xx~&~xx~&~xx~\\
  \bottomrule
  \end{tabular}
  }
\end{table}

==> tabs/abla_diff_modules.tex <==
\begin{table}[tb]
  \caption{Ablation study on different modules of our 2D-3D fusion pipeline.}
  \label{tab:abla_modules}
  \setlength{\tabcolsep}{5pt}
  \renewcommand{\arraystretch}{1}
  \centering
  \resizebox{\columnwidth}{!}{
  \begin{tabular}{cc|ccc|ccc}
    \toprule
    \multicolumn{2}{c|}{Image Features} & \multicolumn{3}{c|}{3DMatch} & \multicolumn{3}{c}{3DLoMatch} \\
    \cline{3-8}
    Pixel-wise~&~Patch-wise~&~FMR(\%)~&~IR(\%)~&~RR(\%)~&~FMR(\%)~&~IR(\%)~&~RR(\%)~\\
    \midrule
    ~&&~97.9~&~71.9~&~92.0~~~&~~88.3~&~43.5~&~74.0~\\
    \checkmark~&~&~\underline{98.8}~&~\textBF{76.2}~&~\underline{94.2}~~~&~~90.1~&~\textBF{48.2}~&~\underline{78.0}~\\    
    ~&~\checkmark~&~98.3~&~68.7~&~91.5~~~&~~92.7~&~40.5~&~77.8~\\
    \checkmark~&~\checkmark~&~\textBF{99.5}~&~\underline{74.3}~&~\textBF{95.9}~~~&~~\textBF{93.6}~&~\textBF{47.4}~&~\textBF{81.6}~\\
  \bottomrule
  \end{tabular}
  }
\end{table}

==> tabs/abla_wo_ransac.tex <==
\begin{table}[tb]
  \caption{Quantitative results with different estimator on 3DMatch and 3DLoMatch datasets. We follow GeoTransformer~\cite{qin2022geometric} to use 5000, 250, and all samples for RANSAC-50k, weighted SVD, LGR estimators, respectively.\andreas{As in all other tables: statistics missing for indicating the uncertainty.}}
  \label{tab:abla_ransac}
  \centering
  \begin{tabular}{l|c|cc}
    \toprule
    \multirow{2}{*}{Method} & \multirow{2}{*}{Estimator} & \multicolumn{2}{c}{RR(\%)} \\
    % \midrule
    % &&&& \\
    & & 3DMatch & 3DLoMatch \\
    \midrule
    \midrule
    FCGF~\cite{FCGF2019}~&\multirow{8}{*}{~RANSAC-50k~}&~85.1~&~40.1~\\
    D3Feat~\cite{bai2020d3feat}~&&~81.6~&~37.2~\\    
    SpinNet~\cite{ao2020SpinNet}~&&~88.6~&~59.8~\\    
    Predator~\cite{predator2021}~&&~89.0~&~59.8~\\
    CoFiNet~\cite{yu2021cofinet}~&&~89.3~&~67.5~\\    
    GeoTransformer~\cite{qin2022geometric}~&&~92.0~&~75.0~\\   
    % PEAL-3D~&&~\textBF{93.0}~&~\textBF{74.2}~\\
    SIRA-PCR~\cite{SIRA_PCR_2023_ICCV}~&&~93.6~&~73.5~\\    
    Ours~&&~\textBF{94.6}~&~\textBF{76.6}~\\
    \midrule
    FCGF~\cite{FCGF2019}~&\multirow{8}{*}{~Weighted SVD~}&~42.1~&~3.9~\\
    D3Feat~\cite{bai2020d3feat}~&&~37.4~&~2.8~\\    
    SpinNet~\cite{ao2020SpinNet}~&&~34.0~&~2.5~\\    
    Predator~\cite{predator2021}~&&~50.0~&~6.4~\\
    CoFiNet~\cite{yu2021cofinet}~&&~64.6~&~21.6~\\    
    GeoTransformer~\cite{qin2022geometric}~&&~86.5~&~59.9~\\    
    % PEAL-3D~&&~\textBF{90.8}~&~\textBF{68.0}~\\
    SIRA-PCR~\cite{SIRA_PCR_2023_ICCV}~&&~89.8~&~64.6~\\  
    Ours~&&~\textBF{90.4}~&~\textBF{66.5}~\\
    \midrule
    CoFiNet~\cite{yu2021cofinet}~&\multirow{4}{*}{~LGR~\cite{qin2022geometric}~}&~87.6~&~64.8~\\
    GeoTransformer~\cite{qin2022geometric}~&&~91.5~&~74.0~\\ 
    % PEAL-3D~&&~\textBF{94.0}~&~\textBF{79.5}~\\
    SIRA-PCR~\cite{SIRA_PCR_2023_ICCV}~&&~94.1~&~76.6~\\    
    Ours~&&~\textBF{95.9}~&~\textBF{81.6}~\\  
  \bottomrule
  \end{tabular}
\end{table}

==> tabs/sup_detailed_3dmatch.tex <==
\begin{table}[tb]
  \caption{Detailed registration results on 3DMatch and 3DLoMatch datasets.}
  \label{tab:scene_regist}
  \setlength{\tabcolsep}{1.5pt}
  \renewcommand{\arraystretch}{1.2}
  \centering
  \resizebox{\columnwidth}{!}{
  \begin{tabular}{l|ccccccccc|ccccccccc}
  \toprule
  \multirow{2}{*}{Method} & \multicolumn{9}{c|}{3DMatch} & \multicolumn{9}{c}{3DLoMatch} \\
   & Kitchen & Home\_1 & Home\_2 & Hotel\_1 & Hotel\_2 & Hotel\_3 & Study & Lab & Avg. & Kitchen & Home\_1 & Home\_2 & Hotel\_1 & Hotel\_2 & Hotel\_3 & Study & Lab & Avg. \\
    \midrule
    % Registration Recall
    \multicolumn{19}{c}{\emph{Registration Recall} (\%) $\uparrow$} \\
    \midrule
    FCGF~\cite{choy2019fully} & \underline{98.0} & 94.3 & 68.6 & 96.7 & \underline{91.0} & \underline{84.6} & 76.1 & 71.1 & 85.1 & 60.8 & 42.2 & 53.6 & 53.1 & 38.0 & 26.8 & 16.1 & 30.4 & 40.1 \\
    D3Feat~\cite{bai2020d3feat} & 96.0 & 86.8 & 67.3 & 90.7 & 88.5 & 80.8 & 78.2 & 64.4 & 81.6 & 49.7 & 37.2 & 47.3 & 47.8 & 36.5 & 31.7 & 15.7 & 31.9 & 37.2 \\
    Predator~\cite{huang2021predator} & 97.6 & \underline{97.2} & \underline{74.8} & \textBF{98.9} & \textBF{96.2} & \textBF{88.5} & 85.9 & 73.3 & 89.0 & 71.5 & 58.2 & 60.8 & 77.5 & 64.2 & 61.0 & 45.8 & 39.1 & 59.8 \\
    GeoTrans~& \textBF{98.9} & \underline{97.2} & \textBF{81.1} & \textBF{98.9} & 89.7 & \textBF{88.5} & \underline{88.9} & \textBF{88.9} & \textBF{91.5} & \textBF{85.9} & \textBF{73.5} & \textBF{72.5} & \textBF{89.5} & \textBF{73.2} & \textBF{66.7} & \textBF{55.3} & \textBF{75.7} & \textBF{74.0} \\
    Ours~& \textBF{99.1} & \underline{99.1} & \textBF{81.8} & \textBF{99.5} & 96.2 & \textBF{100} & \underline{96.2} & \textBF{95.6} & \textBF{95.9} & \textBF{88.0} & \textBF{79.2} & \textBF{79.7} & \textBF{92.9} & \textBF{82.6} & \textBF{73.8} & \textBF{75.1} & \textBF{81.4} & \textBF{81.6} \\
    \midrule
    % Relative Rotation Error
    \multicolumn{19}{c}{\emph{Relative Rotation Error} ($^{\circ}$) $\downarrow$} \\
    \midrule
    FCGF~\cite{choy2019fully} & \textBF{1.767} & 1.849 & \underline{2.210} & 1.867 & 1.667 & 2.417 & \underline{2.024} & \underline{1.792} & \underline{1.949} & \underline{2.904} & 3.229 & 3.277 & 2.768 & \underline{2.801} & \underline{2.822} & 3.372 & 4.006 & 3.147 \\
    D3Feat~\cite{bai2020d3feat} & 2.016 & 2.029 & 2.425 & 1.990 & 1.967 & 2.400 & 2.346 & 2.115 & 2.161 & 3.226 & 3.492 & 3.373 & 3.330 & 3.165 & 2.972 & 3.708 & 3.619 & 3.361 \\
    Predator~\cite{huang2021predator} & 1.861 & \underline{1.806} & 2.473 & 2.045 & \underline{1.600} & 2.458 & 2.067 & 1.926 & 2.029 & 3.079 & \underline{2.637} & \underline{3.220} & \underline{2.694} & 2.907 & 3.390 & \underline{3.046} & 3.412 & \underline{3.048} \\
    GeoTrans~& \underline{1.797} & \textBF{1.353} & \textBF{1.797} & \textBF{1.528} & \textBF{1.328} & \textBF{1.571} & \textBF{1.952} & \textBF{1.678} & \textBF{1.625} & \textBF{2.356} & \textBF{2.305} & \textBF{2.541} & \textBF{2.455} & \textBF{2.490} & \textBF{2.504} & \textBF{3.010} & \textBF{2.716} & \textBF{2.547} \\
    Ours~& \underline{1.929} & \textBF{1.501} & \textBF{1.821} & \textBF{1.716} & \textBF{1.362} & \textBF{1.839} & \textBF{1.875} & \textBF{1.690} & \textBF{1.717} & \textBF{2.635} & \textBF{2.181} & \textBF{2.860} & \textBF{2.668} & \textBF{2.520} & \textBF{2.502} & \textBF{2.667} & \textBF{2.934} & \textBF{2.621} \\
    \midrule
    % Relative Translation Error
    \multicolumn{19}{c}{\emph{Relative Translation Error} (m) $\downarrow$} \\
    \midrule
    FCGF~\cite{choy2019fully} & 0.053 & 0.056 & 0.071 & \underline{0.062} & 0.061 & 0.055 & 0.082 & 0.090 & 0.066 & 0.084 & 0.097 & \underline{0.076} & 0.101 & 0.084 & 0.077 & 0.144 & 0.140 & 0.100 \\
    D3Feat~\cite{bai2020d3feat} & 0.055 & 0.065 & 0.080 & 0.064 & 0.078 & \underline{0.049} & 0.083 & 0.064 & 0.067 & 0.088 & 0.101 & 0.086 & \underline{0.099} & 0.092 & \underline{0.075} & 0.146 & 0.135 & 0.103 \\
    Predator~\cite{huang2021predator} & 0.048 & \underline{0.055} & 0.070 & 0.073 & 0.060 & 0.065 & \underline{0.080} & \underline{0.063} & 0.064 & 0.081 & 0.080 & 0.084 & \underline{0.099} & 0.096 & 0.077 & \textBF{0.101} & 0.130 & \underline{0.093} \\
    GeoTrans~& \textBF{0.042} & \textBF{0.046} & \textBF{0.059} & \textBF{0.055} & \textBF{0.046} & 0.050 & \textBF{0.073} & \textBF{0.053} & \textBF{0.053} & \textBF{0.062} & \textBF{0.070} & \textBF{0.071} & \textBF{0.080} & \textBF{0.075} & \textBF{0.049} & \underline{0.107} & \textBF{0.083} & \textBF{0.074} \\
    Ours~& \textBF{0.046} & \textBF{0.047} & \textBF{0.058} & \textBF{0.058} & \textBF{0.048} & 0.048 & \textBF{0.072} & \textBF{0.052} & \textBF{0.054} & \textBF{0.069} & \textBF{0.066} & \textBF{0.074} & \textBF{0.089} & \textBF{0.070} & \textBF{0.056} & \underline{0.095} & \textBF{0.101} & \textBF{0.078} \\
  \bottomrule
  \end{tabular}
  }
\end{table}
